Homotopy Mackey functors of equivariant algebraic $K$-theory

Given a finite group $G$ acting on a ring $R$, Merling constructed an equivariant algebraic $K$-theory $G$-spectrum, and work of Malkiewich and Merling, as well as work of Barwick, provides an interpretation of this construction as a spectral Mackey functor. This construction is powerful, but highly categorical; as a result the Mackey functors comprising the homotopy are not obvious from the construction and have therefore not yet been calculated. In this work, we provide a computation of the homotopy Mackey functors of equivariant algebraic $K$-theory in terms of a purely algebraic construction. In particular, we construct Mackey functors out of the $n$th algebraic $K$-groups of group rings whose multiplication is twisted by the group action. Restrictions and transfers for these functors admit a tractable algebraic description in that they arise from restriction and extension of scalars along module categories of twisted group rings. In the case where the group action is trivial, our construction recovers work of Dress and Kuku from the 1980's which constructs Mackey functors out of the algebraic $K$-theory of group rings. We develop many families of examples of Mackey functors, both new and old, including $K$-theory of endomorphism rings, the $K$-theory of fixed subrings of Galois extensions, and (topological) Hochschild homology of twisted group rings.

==> commands.tex <==
% Custom Arrows
% 
% (c) Thomas Brazelton
%
%% This program can be redistributed and/or modified under the terms
%% of the LaTeX Project Public License Distributed from CTAN archives
%% in directory macros/latex/base/lppl.txt.
% 

% Packages
\RequirePackage{amsmath,amssymb}
\RequirePackage{amsfonts}
\RequirePackage{geometry}
%\RequirePackage{hyperref}
\RequirePackage{color}
\RequirePackage{mathtools}		% used for arrows
%\RequirePackage{ bbold }
\RequirePackage{bbm}
\RequirePackage{amsfonts}
\RequirePackage{mathrsfs}
\RequirePackage{tikz}
%\usepackage[shortlabels]{enumitem}
\usetikzlibrary{shapes.geometric, arrows}
\usetikzlibrary{decorations.pathmorphing}
\usetikzlibrary{cd}
\tikzstyle{arrow} = [thick,->,>=stealth]


% Arrows
\providecommand{\po}{\arrow[ul,phantom,"\ulcorner" very near start]}
\providecommand{\pb}{\arrow[dr,phantom,"\lrcorner" very near start]}
\providecommand{\pol}{\arrow[ur,phantom,"\urcorner" very near start]}
\providecommand{\pbr}{\arrow[dl,phantom,"\llcorner" very near start]}
\providecommand{\xto}[1]{\xrightarrow{#1}}
\providecommand{\from}{\leftarrow}
\providecommand{\xfrom}[1]{\overset{#1}{\leftarrow}}

\providecommand{\mapsfrom}{\mathrel{\reflectbox{\ensuremath{\mapsto}}}}
\providecommand{\longmapsfrom}{\mathrel{\reflectbox{\ensuremath{\longmapsto}}}}

\providecommand{\hookto}{\xhookrightarrow{}}
\providecommand{\xhookto}[1]{\overset{#1}{\hookrightarrow}}

\providecommand{\hookfrom}{\xhookleftarrow{}}
\providecommand{\xhookfrom}[1]{\xhookleftarrow{#1}}

\providecommand{\tto}{\twoheadrightarrow}
\providecommand{\xtto}[1]{\overset{#1}{\twoheadrightarrow}}
\providecommand{\ffrom}{\twoheadleftarrow}
\providecommand{\xffrom}[1]{\overset{#1}{\ffrom}}

\providecommand{\ladjoint}[2]{ #1\rightleftarrows #2 }
\makeatletter
\providecommand{\superimpose}[2]{%
  {\ooalign{$#1\@firstoftwo#2$\cr\hfil$#1\@secondoftwo#2$\hfil\cr}}}
\makeatother
\providecommand{\smallslash}{\mbox{\tiny/}}

\providecommand{\clhookto}{\mathrel{\raisebox{0.1em}{$\mathrel{\mathpalette\superimpose{{\hspace{0.1cm}\vspace{0.1em}\smallslash}{\hookrightarrow}}}$}}}
\providecommand{\xclhook}[1]{\overset{#1}{\clhook}}

\providecommand{\clhookfrom}{\mathrel{\raisebox{0.1em}{$\mathrel{\mathpalette\superimpose{{\hspace{0.1cm}\vspace{0.1em}\smallslash}{\hookleftarrow}}}$}}}

\providecommand{\ohookto}{\mathrel{\raisebox{0.03em}{$\mathrel{\mathpalette\superimpose{{\hspace{0.1cm}\vspace{0.03em}\mbox{\small$\circ$}}{\hookrightarrow}}}$}}}

\providecommand{\ohookfrom}{\mathrel{\raisebox{0.03em}{$\mathrel{\mathpalette\superimpose{{\hspace{0.1cm}\vspace{0.03em}\mbox{\small$\circ$}}{\hookleftarrow}}}$}}}

\providecommand{\cofto}{\rightarrowtail}
\providecommand{\coffrom}{\leftarrowtail}
\providecommand{\xcofto}[1]{\overset{#1}{\cofto}}
\providecommand{\xcoffrom}[1]{\overset{#1}{\coffrom}}

% Common Text Commands
\providecommand{\ab}{\text{ab}}
\providecommand{\ann}{\text{ann}}
\providecommand{\Arg}{\text{Arg}}
\providecommand{\Aut}{\text{Aut}}

\providecommand{\Bimor}{\text{Bimor}}
\providecommand{\Br}{\text{Br}}

\providecommand{\cl}{\text{cl}}
\providecommand{\codim}{\text{codim}}
\providecommand{\cof}{\text{cof}}
\providecommand{\cofib}{\text{cofib}}
\providecommand{\coker}{\text{coker}}
\providecommand{\colim}{\text{colim}}
\providecommand{\Comm}{\text{Comm}}
\providecommand{\Compl}{\text{Compl}}
\providecommand{\Conf}{\text{Conf}}
\providecommand{\conj}{\text{conj}}
\providecommand{\const}{\text{const}}
\providecommand{\cosk}{\text{cosk}}

\providecommand{\Der}{\text{Der}}
\providecommand{\diam}{\text{diam}}
\providecommand{\Diff}{\text{Diff}}
\providecommand{\disc}{\text{disc}}
\providecommand{\Disc}{\text{Disc}}

\providecommand{\Emb}{\text{Emb}}
\providecommand{\End}{\text{End}}
\providecommand{\Ext}{\text{Ext}}
\providecommand{\et}{\text{\'{e}t}}
\providecommand{\ev}{\text{ev}}

\providecommand{\fib}{\text{fib}}
\providecommand{\Fix}{\text{Fix}}
\providecommand{\Fr}{\text{Fr}}
\providecommand{\Frac}{\text{Frac}}
\providecommand{\Frob}{\text{Frob}}
\providecommand{\Fun}{\text{Fun}}

\providecommand{\Gal}{\text{Gal}}
\providecommand{\GL}{\text{GL}}
\providecommand{\gr}{\text{gr}}

\providecommand{\HH}{\text{HH}}
\providecommand{\hocofib}{\text{hocofib}}
\providecommand{\hocolim}{\text{hocolim}}
\providecommand{\hofib}{\text{hofib}}
\providecommand{\holim}{\text{holim}}
\providecommand{\Hom}{\text{Hom}}

\providecommand{\id}{\text{id}}
\providecommand{\im}{\text{im}}
\renewcommand{\Im}{\text{Im}}
\providecommand{\incl}{\text{incl}}
\providecommand{\ind}{\text{ind}}
\providecommand{\Ind}{\text{Ind}}
\providecommand{\Inn}{\text{Inn}}

\providecommand{\Jac}{\text{Jac}}

\providecommand{\Loc}{\text{Loc}}

\providecommand{\Map}{\text{Map}}
\providecommand{\Mat}{\text{Mat}}
\providecommand{\mor}{\text{mor}}
\providecommand{\mult}{\text{mult}}

\providecommand{\Nis}{\text{Nis}}

\providecommand{\ob}{\text{ob}}
\providecommand{\obj}{\text{obj}}
\providecommand{\op}{\text{op}}
\providecommand{\Orb}{\text{Orb}}
\providecommand{\ord}{\text{ord}}
\providecommand{\Out}{\text{Out}}

\providecommand{\per}{\text{per}}
\providecommand{\Perf}{\text{Perf}}
\providecommand{\Perm}{\text{Perm}}
\providecommand{\Poly}{\text{Poly}}
\providecommand{\pr}{\text{pr}}
\providecommand{\pre}{\text{pre}}
\providecommand{\Prob}{\text{Prob}}
\providecommand{\Proj}{\text{Proj}}
\providecommand{\PGL}{\text{PGL}}
\providecommand{\PSL}{\text{PSL}}

\providecommand{\quot}{\text{quot}}

\providecommand{\rad}{\text{rad}}
\providecommand{\rank}{\text{rank}}
\renewcommand{\Re}{\text{Re}}
\providecommand{\Rep}{\text{Rep}}
\providecommand{\Res}{\text{Res}}
\providecommand{\res}{\text{res}}

\providecommand{\sgn}{\text{sgn}}
\providecommand{\sig}{\text{sig}}
\providecommand{\Sing}{\text{Sing}}
\providecommand{\SL}{\text{SL}}
\providecommand{\SO}{\text{SO}}
\providecommand{\spn}{\text{span}}
\providecommand{\Stab}{\text{Stab}}
\providecommand{\Sub}{\text{Sub}}
\providecommand{\supp}{\text{supp}}
\providecommand{\Syl}{\text{Syl}}
\providecommand{\syl}{\text{syl}}
\providecommand{\Sym}{\text{Sym}}

\providecommand{\Tor}{\text{Tor}}
\providecommand{\Tr}{\text{Tr}}
\providecommand{\tr}{\text{tr}}

\providecommand{\vol}{\text{vol}}

\providecommand{\Zar}{\text{Zar}}


% BB Sets
\providecommand{\C}{\mathbb{C}}
\providecommand{\F}{\mathbb{F}}
\providecommand{\N}{\mathbb{N}}
\providecommand{\Q}{\mathbb{Q}}
\providecommand{\R}{\mathbb{R}}
\providecommand{\Z}{\mathbb{Z}}

% Projective
\newcommand{\CP}{\mathbb{C}\text{P}}
\newcommand{\RP}{\mathbb{R}\text{P}}

% Colors
\providecommand{\green}[1]{\textcolor{green}{#1}}
\providecommand{\red}[1]{\textcolor{red}{#1}}
\providecommand{\orange}[1]{\textcolor{orange}{#1}}
\providecommand{\green}[1]{\textcolor{green}{#1}}
\providecommand{\blue}[1]{\textcolor{blue}{#1}}
\providecommand{\purple}[1]{\textcolor{purple}{#1}}

% Commands
\providecommand{\ceil}[1]{\left\lceil #1 \right\rceil}
\providecommand{\floor}[1]{\left\lfloor #1 \right\rfloor}
\providecommand{\lrangle}[1]{\left\langle #1 \right\rangle}
\providecommand{\und}[1]{\underline{#1}}
\renewcommand{\hat}{\widehat}
\providecommand{\legendre}[2]{\left( \substack{#1 \\ #2} \right)}
\providecommand{\trianglerightneq}{\mathrel{\ooalign{\raisebox{-0.5ex}{\reflectbox{\rotatebox{90}{$\nshortmid$}}}\cr$\triangleright$\cr}\mkern-3mu}}
\providecommand{\triangleleftneq}{\mathrel{\reflectbox{$\trianglerightneq$}}}

% Other
\providecommand{\dot}{\bullet}
\let\oldemptyset\emptyset
\let\emptyset\varnothing
\providecommand{\setminus}{\smallsetminus}
\providecommand{\minus}{\smallsetminus}
\let\bar\overline
\let\tilde\widetilde
\let\til\widetilde
\let\nsubgp\trianglelefteq
\let\del\partial
\let\epsilon\varepsilon
\providecommand{\bigast}{\mathop{\scalebox{1.5}{\raisebox{-0.2ex}{$\ast$}}}}
\providecommand{\llangle}{\left\langle\hspace{-0.2em}\left\langle}
\providecommand{\rrangle}{\right\rangle\hspace{-0.2em}\right\rangle}
\providecommand{\Pfister}[1]{\llangle #1 \rrangle}


% operp command for quadratic forms, from mathabx.sty
% https://tex.stackexchange.com/a/61882/
\DeclareFontFamily{U}{matha}{\hyphenchar\font45}
\DeclareFontShape{U}{matha}{m}{n}{
      <5> <6> <7> <8> <9> <10> gen * matha
      <10.95> matha10 <12> <14.4> <17.28> <20.74> <24.88> matha12
      }{}
\DeclareSymbolFont{matha}{U}{matha}{m}{n}
\DeclareFontFamily{U}{mathx}{\hyphenchar\font45}
\DeclareFontShape{U}{mathx}{m}{n}{
      <5> <6> <7> <8> <9> <10>
      <10.95> <12> <14.4> <17.28> <20.74> <24.88>
      mathx10
      }{}
\DeclareSymbolFont{mathx}{U}{mathx}{m}{n}
\DeclareMathSymbol{\operp}         {2}{matha}{"6B}
\DeclareMathSymbol{\bigoperp}       {1}{mathx}{"CB}



\RequirePackage{amsmath,amssymb}
\RequirePackage{geometry}

% AG commands
\providecommand{\Aut}{\text{Aut}}
\providecommand{\B}{\text{B}}
\providecommand{\Bez}{\text{B\'ez}}
\providecommand{\BGL}{\text{BGL}}
\providecommand{\Bl}{\text{Bl}}
\providecommand{\CH}{\text{CH}}
\providecommand{\char}{\text{char}}
\providecommand{\cof}{\text{cof}}
\providecommand{\Coker}{\text{Coker}}
\providecommand{\coker}{\text{coker}}
\providecommand{\colim}{\text{colim}}
\providecommand{\Disc}{\text{Disc}}
\providecommand{\EKL}{\text{EKL}}
\providecommand{\End}{\text{End}}
\providecommand{\et}{\text{\'{e}t}}
\providecommand{\Fix}{\text{Fix}}
\providecommand{\Frac}{\text{Frac}}
\providecommand{\Frob}{\text{Frob}}
\providecommand{\Fun}{\text{Fun}}
\providecommand{\GL}{\text{GL}}
\providecommand{\GW}{\text{GW}}
\providecommand{\Gr}{\text{Gr}}
\providecommand{\grad}{\text{grad}}
\providecommand{\Hom}{\text{Hom}}
\providecommand{\Im}{\text{Im}}
\providecommand{\Jac}{\text{Jac}}
\providecommand{\K}{\mathcal{K}}
\providecommand{\Ker}{\text{Ker}}
\providecommand{\Map}{\text{Map}}
\providecommand{\MW}{\text{MW}}
\providecommand{\Nis}{\text{Nis}}
\providecommand{\op}{\text{op}}
\providecommand{\Pic}{\text{Pic}}
\providecommand{\Pre}{\text{Pre}}
\providecommand{\Proj}{\text{Proj}\hspace{0.1em}}
\providecommand{\PSL}{\text{PSL}}
\providecommand{\rank}{\text{rank}}
\providecommand{\Rep}{\text{Rep}}
\providecommand{\Res}{\text{Res}}
\providecommand{\s}{\text{s}}
\providecommand{\sgn}{\text{sgn}}
\providecommand{\Sh}{\text{Sh}}
\providecommand{\sig}{\text{sig}}
\providecommand{\Sm}{\textit{Sm}}
\providecommand{\SO}{\text{SO}}
\providecommand{\Sp}{\text{Sp}}
\providecommand{\Spc}{\text{Spc}}
\providecommand{\Spec}{\text{Spec}\hspace{0.1em}}
\providecommand{\Spin}{\text{Spin}}
\providecommand{\sSet}{\textit{sSet}}
\providecommand{\SU}{\text{SU}}
\providecommand{\supp}{\text{supp}}
\providecommand{\Sym}{\text{Sym}}

\providecommand{\Th}{\text{Th}}
\providecommand{\Tr}{\text{Tr}}
\providecommand{\type}{\text{type}}
\providecommand{\Wr}{\text{Wr}}


\providecommand{\O}{\mathcal{O}}
\providecommand{\H}{\textbf{H}}
% AG Categories
\providecommand{\Aff}{\textit{Aff}}
\providecommand{\AffVar}{\textit{AffVar}}
\providecommand{\Sch}{\textit{Sch}}
\providecommand{\preVar}[1]{\textit{preVar}\text{-}#1}
% AG Symbols
\providecommand{\A}{\mathbb{A}}
\providecommand{\G}{\mathbb{G}}
\providecommand{\Gm}{\mathbb{G}_{\text{m}}}
\renewcommand{\H}{\mathbb{H}}

\providecommand{\m}{\mathfrak{m}}
\renewcommand{\O}{\mathscr{O}}
\providecommand{\p}{\mathfrak{p}}
\renewcommand{\P}{\mathbb{P}}
\providecommand{\q}{\mathfrak{q}}

\newcommand{\gw}[1]{\left\langle #1 \right\rangle}


% AG Arrows
\providecommand{\dashto}{\dashrightarrow}
\providecommand{\dashfrom}{\mathrel{\reflectbox{\ensuremath{\dashrightarrow}}}}

\RequirePackage{amsmath,amssymb}
\RequirePackage{geometry}

% AT commands
\providecommand{\BG}{\text{BG}}
\providecommand{\BO}{\text{BO}}
\providecommand{\BU}{\text{BU}}
\providecommand{\BSO}{\text{BSO}}
\providecommand{\BSU}{\text{BSU}}
\providecommand{\BGL}{\text{BGL}}
\providecommand{\coeq}{\text{coeq}}
\providecommand{\cof}{\text{cof}}
\providecommand{\cone}{\text{cone}}
\providecommand{\eq}{\text{eq}}
\providecommand{\Ext}{\text{Ext}}
\providecommand{\Gr}{\text{Gr}}
\providecommand{\Ho}{\text{Ho}}
\providecommand{\hocofib}{\text{hocofib}}
\providecommand{\hocolim}{\text{hocolim}}
\providecommand{\holim}{\text{holim}}
\providecommand{\KO}{\text{KO}}
\providecommand{\KR}{\text{KR}}
\providecommand{\KU}{\text{KU}}
\providecommand{\Lan}{\text{Lan}}
\providecommand{\MGL}{\text{MGL}}
\providecommand{\MO}{\text{MO}}
\providecommand{\MSO}{\text{MSO}}
\providecommand{\MU}{\text{MU}}
\providecommand{\Out}{\text{Out}}
\providecommand{\pre}{\text{pre}}
\providecommand{\Ran}{\text{Ran}}
\providecommand{\RO}{\text{RO}}
\providecommand{\Sing}{\text{Sing}}
\providecommand{\SO}{\text{SO}}
\providecommand{\SU}{\text{SU}}
\providecommand{\Sym}{\text{Sym}}
\providecommand{\Th}{\text{Th}}


\providecommand{\Sp}{\textit{Sp}}

% Spaces
\providecommand{\CP}{\mathbb{C}\text{P}}
\providecommand{\HP}{\mathbb{H}\text{P}}
\providecommand{\RP}{\mathbb{R}\text{P}}

% Other
\providecommand{\Cech}{\check{C}}
\let\adj\dashv


\RequirePackage{amsmath,amssymb,amsfonts}
\RequirePackage{bbm}


% Categories
\providecommand{\onecat}{\mathbbm{1}}
\providecommand{\twocat}{\mathbbm{2}}
\providecommand{\Alg}{\texttt{Alg}}
\providecommand{\Ab}{\texttt{Ab}}
\providecommand{\Cat}{\texttt{Cat}}
\providecommand{\CDGA}{\texttt{CDGA}}
\providecommand{\CG}{\texttt{CG}}
\providecommand{\CGWH}{\texttt{CGWH}}
\providecommand{\Ch}{\texttt{Ch}}
\providecommand{\Coh}{\texttt{Coh}}
\providecommand{\CommRing}{\texttt{CommRing}}
\providecommand{\Corr}{\texttt{Corr}}
\providecommand{\CRing}{\texttt{CRing}}
\providecommand{\CW}{\texttt{CW}}
\providecommand{\Field}{\texttt{Field}}
\providecommand{\Grp}{\texttt{Grp}}
\providecommand{\Grpd}{\texttt{Grpd}}
\providecommand{\Grph}{\texttt{Grph}}
\providecommand{\Kar}{\texttt{Kar}}
\providecommand{\Kan}{\texttt{Kan}}
\providecommand{\Mod}{\texttt{Mod}}
\providecommand{\lmod}[1]{#1\text{-}\texttt{Mod}}
\providecommand{\rmod}[1]{\texttt{Mod}\text{-}#1}
\providecommand{\bimod}[2]{#1\text{-}\texttt{Mod}\text{-}#2}
\providecommand{\Ouv}{\texttt{Ouv}}
\providecommand{\Poset}{\texttt{Poset}}
\providecommand{\qCat}{\texttt{qCat}}
\providecommand{\QCoh}{\texttt{QCoh}}
\providecommand{\Ring}{\texttt{Ring}}
\providecommand{\Set}{\texttt{Set}}
\providecommand{\Spectra}{\texttt{Spectra}}
\providecommand{\sSet}{\texttt{sSet}}
\providecommand{\Top}{\texttt{Top}}
\providecommand{\Ring}{\texttt{Ring}}
\providecommand{\Vect}{\texttt{Vect}}

% Other
\providecommand{\dg}{\text{dg}}
\providecommand{\inj}{\text{inj}}
\providecommand{\mor}{\text{mor}}
\providecommand{\Mor}{\text{Mor}}
\providecommand{\ob}{\text{ob}}
\providecommand{\obj}{\text{obj}}
\providecommand{\proj}{\text{proj}}


\newcommand{\DDelta}{\bm{\Delta}}


% Limits
\providecommand{\llim}{\varprojlim}
\providecommand{\rlim}{\varinjlim}



%%
%% End of file `custom-arrows.sty'.

